Direct Preference Optimization of Video Large Multimodal Models from Language Model Reward

Preference modeling techniques, such as direct preference optimization (DPO), has shown effective in enhancing the generalization abilities of large language model (LLM). However, in tasks involving video instruction-following, providing informative feedback, especially for detecting hallucinations in generated responses, remains a significant challenge. Previous studies have explored using large large multimodal models (LMMs) as reward models to guide preference modeling, but their ability to accurately assess the factuality of generated responses compared to corresponding videos has not been conclusively established. This paper introduces a novel framework that utilizes detailed video captions as a proxy of video content, enabling language models to incorporate this information as supporting evidence for scoring video Question Answering (QA) predictions. Our approach demonstrates robust alignment with OpenAI GPT-4V model's reward mechanism, which directly takes video frames as input. Furthermore, we show that applying this tailored reward through DPO significantly improves the performance of video LMMs on video QA tasks.

==> tex/094_hyperparam.tex <==
\begin{figure}[t]
\centering
\small
\centering
\begin{minted}[fontsize=\footnotesize, frame=single,linenos=false,breaklines,breaksymbol=,escapeinside=||,bgcolor=Box3Color]{bash}
# actual batch size is 8 x 16=128
torchrun --nproc_per_node=8 --master_port=$port llava/train/train_mem.py \
    --deepspeed ./scripts/zero2.json \
    --model_name_or_path $model_name_or_path \
    --version v1 \
    --data_paths $data_paths --sample_ratios $sample_ratios \
    --video_folder $video_dir \
    --image_folder $image_dir \
    --X "Video" "Image" \
    --video_tower LanguageBind/LanguageBind_Video_merge \
    --image_tower LanguageBind/LanguageBind_Image \
    --pretrain_mm_mlp_adapter $mm_adapter_path \
    --mm_projector_type mlp2x_gelu \
    --mm_vision_select_layer -2 \
    --mm_use_x_start_end False \
    --mm_use_x_patch_token False \
    --image_aspect_ratio pad \
    --group_by_modality_length False \
    --bf16 True \
    --output_dir $output_dir \
    --num_train_epochs 1 \
    --per_device_train_batch_size 16 \
    --per_device_eval_batch_size 4 \
    --gradient_accumulation_steps 1 \
    --evaluation_strategy "no" \
    --save_strategy "steps" \
    --save_only_model True \
    --learning_rate 2e-5 \
    --weight_decay 0. \
    --warmup_ratio 0.03 \
    --lr_scheduler_type "cosine" \
    --logging_steps 1 \
    --tf32 True \
    --model_max_length 2048 \
    --gradient_checkpointing True \
    --dataloader_num_workers 8 \
    --lazy_preprocess True \
    --cache_dir $cache_dir
\end{minted}
\caption{Hyperparameters for pre-training stage.}
\label{fig:hyperparam_pretrain}
\end{figure}


\begin{figure}[t]
\centering
\small
\centering
\begin{minted}[fontsize=\footnotesize, frame=single,linenos=false,breaklines,breaksymbol=,escapeinside=||,bgcolor=Box3Color]{bash}
# actual batch size is 8 x 16=128
torchrun --nproc_per_node=8 --master_port=$port llava/train/train_mem.py \
    --deepspeed ./scripts/zero2.json \
    --model_name_or_path $model_name_or_path \
    --version v1 \
    --data_path $data_path \
    --video_folder $video_dir \
    --image_folder $image_dir \
    --X "Video" "Image" \
    --video_tower LanguageBind/LanguageBind_Video_merge \
    --image_tower LanguageBind/LanguageBind_Image \
    --mm_projector_type mlp2x_gelu \
    --mm_vision_select_layer -2 \
    --mm_use_x_start_end False \
    --mm_use_x_patch_token False \
    --image_aspect_ratio pad \
    --group_by_modality_length False \
    --bf16 True \
    --output_dir $output_dir \
    --num_train_epochs 1 \
    --per_device_train_batch_size 16 \
    --per_device_eval_batch_size 4 \
    --gradient_accumulation_steps 1 \
    --evaluation_strategy "no" \
    --save_strategy "steps" \
    --save_steps 2000 \
    --save_only_model True \
    --save_total_limit 5 \
    --learning_rate 5e-6 \
    --weight_decay 0. \
    --warmup_ratio 0.03 \
    --lr_scheduler_type "cosine" \
    --logging_steps 1 \
    --tf32 True \
    --model_max_length 2048 \
    --gradient_checkpointing True \
    --dataloader_num_workers 8 \
    --lazy_preprocess True \
    --report_to wandb \
    --cache_dir $cache_dir 2>&1 | tee $output_dir/train.log
\end{minted}
\caption{Hyperparameters for fine-tuning stage.}
\label{fig:hyperparam_finetune}
\end{figure}


\begin{figure}[t]
\centering
\small
\centering
\begin{minted}[fontsize=\footnotesize, frame=single,linenos=false,breaklines,breaksymbol=,escapeinside=||,bgcolor=Box3Color]{bash}
# actual batch size is 8 x 16=128
torchrun --nproc_per_node=8 --master_port=$port llava/train/train_mem.py \
    --deepspeed /mnt/bn/liangkeg/ruohongz/vllm/scripts/zero2.json \
    --model_name_or_path $model_name_or_path \
    --version v1 \
    --data_path $data_path \
    --video_folder $video_dir \
    --image_folder $image_dir \
    --X "Video" "Image" \
    --video_tower LanguageBind/LanguageBind_Video_merge \
    --image_tower LanguageBind/LanguageBind_Image \
    --mm_projector_type mlp2x_gelu \
    --mm_vision_select_layer -2 \
    --mm_use_x_start_end False \
    --mm_use_x_patch_token False \
    --image_aspect_ratio pad \
    --group_by_modality_length False \
    --bf16 True \
    --output_dir $output_dir \
    --num_train_epochs 1 \
    --per_device_train_batch_size 16 \
    --per_device_eval_batch_size 4 \
    --gradient_accumulation_steps 1 \
    --evaluation_strategy "no" \
    --save_strategy "steps" \
    --save_steps 2000 \
    --save_only_model True \
    --save_total_limit 5 \
    --learning_rate 5e-6 \
    --weight_decay 0. \
    --warmup_ratio 0.03 \
    --lr_scheduler_type "cosine" \
    --logging_steps 1 \
    --tf32 True \
    --model_max_length 2048 \
    --gradient_checkpointing True \
    --dataloader_num_workers 8 \
    --lazy_preprocess True \
    --report_to wandb \
    --cache_dir $cache_dir 2>&1 | tee $output_dir/train.log
\end{minted}
\caption{Hyperparameters for fine-tuning stage.}
\label{fig:hyperparam_finetune}
\end{figure}

==> tex/tmp.tex <==
\begin{table}[ht]
    \centering
    \begin{tabular}{c | c c}
    \toprule
    & 7b & 13b \\
    \midrule
    500k & 54.85 & 53.66 \\
    50k & 44.44 & 43.38 \\
    GPT-4V & \multicolumn{2}{c}{61.58} \\
    \bottomrule
    \end{tabular}
    \caption{Number of distillation data vs. captioning ability.}
    \label{tab:eval_distillation}
\end{table}

\begin{table}[ht]
    \centering
    \begin{tabular}{c | c c c }
    \toprule
    & 10\% & 40\% & 60\% \\
    \midrule
    SFT captioner & 44.44 & 48.70 & 46.57 \\
    self-trained captioner & 42.67 & 48.23 & 48.94 \\
    \bottomrule
    \end{tabular}
    \caption{Effectiveness of self-labeling and self-training.}
    \label{tab:eval_selftrain}
\end{table}

\begin{figure}[t!]
    \centering
    \includegraphics[width=0.8\linewidth]{fig/caption_trend.pdf}
    \caption{Trend of video-captioning ability vs. number of distilled data.}
    \label{fig:caption_trend}
\end{figure}

